SLUGGER: Lossless Hierarchical Summarization of Massive Graphs

Given a massive graph, how can we exploit its hierarchical structure for concisely but exactly summarizing the graph? By exploiting the structure, can we achieve better compression rates than state-of-the-art graph summarization methods? The explosive proliferation of the Web has accelerated the emergence of large graphs, such as online social networks and hyperlink networks. Consequently, graph compression has become increasingly important to process such large graphs without expensive I/O over the network or to disk. Among a number of approaches, graph summarization, which in essence combines similar nodes into a supernode and describe their connectivity concisely, protrudes with several advantages. However, we note that it fails to exploit pervasive hierarchical structures of real-world graphs as its underlying representation model enforces supernodes to be disjoint. In this work, we propose the hierarchical graph summarization model, which is an expressive graph representation model that includes the previous one proposed by Navlakha et al. as a special case. The new model represents an unweighted graph using positive and negative edges between hierarchical supernodes, each of which can contain others. Then, we propose Slugger, a scalable heuristic for concisely and exactly representing a given graph under our new model. Slugger greedily merges nodes into supernodes while maintaining and exploiting their hierarchy, which is later pruned. Slugger significantly accelerates this process by sampling, approximation, and memoization. Our experiments on 16 real-world graphs show that Slugger is (a) Effective: yielding up to 29.6% more concise summary than state-of-the-art lossless summarization methods, (b) Fast: summarizing a graph with 0.8 billion edges in a few hours, and (c) Scalable: scaling linearly with the number of edges in the input graph.

==> 02_Problem_Definition_old.tex <==
\section{Hierarchical Graph Model}
\label{sec:preliminaries}
\begin{figure*}[t]
	\vspace{-6mm}
	\centering
	\subfigure[$O(nk)$]{
		\label{inputgraph}
		\includegraphics[width= 0.23\linewidth]{./fig/figure1.pdf}
	} 
	\subfigure[$O(nk^2)$]{
		\label{adj}
		\includegraphics[width= 0.23\linewidth]{./fig/figure2.pdf}
	} 
	\subfigure[$O(n^2 + nk)$]{
		\label{summarygraph}
		\includegraphics[width= 0.23\linewidth]{./fig/figure3.pdf}
	} 
	\subfigure[$O(n^2k^2)$]{
		\label{readj}
		\includegraphics[width= 0.23\linewidth]{./fig/figure4.pdf}
	} \\ \vspace{-2mm}
	\caption{\label{fig:concept} 
		\underline{\smash{Hierarchical graph model gives a concise representation.}} The total encoding cost of the given hierarchical model $\overline{G}$ in (a) has $O(nk)$, where $n$ is a number of nodes excluding subnodes (or leaf nodes) and $k$ is the number of subnodes that belongs to each node. Note that the previous model can represent the input graph in one of the three possibilities, which are (b), (c), or (d).  
	}
\end{figure*}

\begin{figure*}[t]
	\vspace{-3mm}
	\centering
	\includegraphics[width= \linewidth]{./fig/figure22.pdf}
	\caption{\label{fig:model} 
		\underline{\smash{Hierarchical graph model}}  
	}
\end{figure*}

\begin{table}[t]
	\vspace{-5mm}
	\small
	\begin{center}
		\caption{Symbols and Definitions.}
		\label{tab:symndef}
		\scalebox{0.9}{
			\begin{tabular}{l|l}
				\toprule 
				\textbf{Symbol}  & \textbf{Definition}\\
				\midrule
				\multicolumn{2}{l}{\bf Symbols for the problem definition (Sect.~\ref{sec:preliminaries})} \\
				\midrule 
				\original & input graph with subnodes $V$ and subedges $E$\\
				$A$ & adjacency matrix of $G$\\
				\midrule
				\sG & hierarchical summary graph with nodes \sN, \\
				&positive edges \pP, negative edges \pM,\\
				&and hierarchy edges \hieredge\\
				$S_X$ & set of leaf nodes in node X, considering X as a rooted tree \\
				\rootS & set of root nodes \\
				$\hat{A}$ & reconstructed adjacency matrix of $\overline{G}$\\
				\midrule
				\summary & summary graph with supernodes \supnode and superedges \supedge\\
				\correction & subedge corrections \\
				$C^+$ & set of subedges to be inserted \\
				$C^-$ & set of subedges to be removed \\ 
				\midrule
				\multicolumn{2}{l}{\bf Symbols for the proposed algorithm (Sect. \ref{sec:method})} \\
				\midrule  
				$T$  &  given number of iterations\\ 
				$\theta(t)$  &  threshold at the $t$-th iteration\\
				$C_t$ &set of candidate sets at the $t$-th iteration\\   
				\bottomrule
			\end{tabular}
		}
	\end{center}
\end{table}

In this section, we introduce graph summarization models, their notations and concepts that are covered throughout the paper first. Then, we formally define the hierarchical graph summarization problem, which extends the previous problem \cite{navlakha2008graph}.
\subsection{Graph Representation Models}
\label{sec:pfn:concept}

\smallsection{Input graph:} We consider an input graph \original as an undirected graph without self-loops (i.e.,$\{\{u, v\} \in E : u \neq v \in V\}$).  Note that modifying our ideas to directed graphs with self-loops is simple but excluded for a clear explanation. We call nodes and edges in $G$ subnodes and subedges, respectively, to avoid confusion with the summary graph's definition below. \label{def:original}

\smallsection{Summary graph:} A summary graph of \original, denoted by \summary, consist of a set of nodes \sN where node set is a partition of $V$ (i.e., $\bigcup_{A \in S} A = V$ and $A \cap B = \emptyset$ for all $A \neq B \in S$), and set of edges $P$ (i.e., $\{\{A, B\} \in P : A, B \in S\}$). We call nodes and edges in $\tilde{G}$ supernodes and superedges, respectively to avoid confusion. In addition, correction \correction consists of sets of edges $C^+$ and $C^-$, which connects a pair of subnodes (i.e., $\{\{u,v\} \in C^+, C^-: u \neq v \in V\}$). Superedge $\{A, B\} \in P$ indicates the connection of all subnode pairs that belong to each $A$ and $B$ with just a single edge. For subedges $\{u, v\} \in E$ but not yet represented with $P$, the model represents them with $C^+$. For subedges $\{u, v\} \notin E$ but represented with $P$, the model save those subedges in $C^-$ for later correction.




\smallsection{Hierarchical summary graph:} A hierarchical summary graph of \original, denoted by \sG, consists of a set of nodes \sN, sets of edges (i.e., positive edges \pP and negative edges \pM), and a set of hierarchy edges \hieredge. We call positive edges p-edges, negative edges n-edges for simplicity. 

Unlike the previous graph summarization model \cite{navlakha2008graph}, subnode $v \in V$ can belong to more than one nodes, allowing the input graph to be expressed with a more diverse connection between nodes. A hierarchy between nodes allows obtaining subnodes belonging to each node from the summary graph itself.\footnote{Note that h-edges \hieredge are also needed in the previous graph summarization problem \cite{navlakha2008graph}, since each supernodes' membership information is not obtainable without them.} Nodes in the hierarchical summary graph thus divide into three parts (a) leaf node, (b) internal node, and (c) root node, where leaf nodes are subnodes (i.e., $v \in V$), root nodes are nodes without parent nodes, and others are internal nodes.
Subnode that belongs to each node $X \in S$ is a set of leaf descendants of a tree with itself as root. We denote $S_X \in V$ as a set of leaf descendants of node $X \in S$ (i.e., $S_X = \{\{l\} : l ~\text{is a leaf nodes in tree}~ X\}$). Thus, the parent node includes all subnodes belonging to its descendent node.
The tree edges constituting the hierarchy between nodes are hierarchy edges \hieredge (i.e., h-edges), connecting each node and its parents. Leaf nodes that do not have parent nodes are considered root nodes. Thus, they don't have a hierarchy at all.

The p-edges \pP and n-edges \pM are sets of pairs of nodes (i.e., $\{\{X, Y\} \in P^+ \cup P^- : X \in S, Y \in S\}$), indicating a positive or negative connection between $S_X$ and $S_Y$. 
Moreover, h-edges \hieredge enables partial decompression (retrieving neighborhood information of particular subnode $v \in V$, without fully reconstructing the original graph) of the original graph \original (see \red{Appendix. \ref{append:query}}). 

\smallsection{Restoring the input graph:} Let $A = |V| \times |V|$ be the adjacency matrix of \original, where the matrix has elements $a_{ij} = 1$ if there is an edge between node $i, j \in V$, and $a_{ij} = 0$ if not. Similarly, let $\hat{A} = |V| \times |V|$ be the reconstructed adjacency matrix of \sG, where $\hat{a}_{ij}$ have an identical value with $a_{ij}$, respect to the same indices. Each elements $(i, j)$ of reconstructed adjacency matrix $\hat{A}$ is computed as follows:
\begin{equation}
\hat{a}_{ij}:=\left\{
\begin{array}{ll}
|\{\{A,B\}\in P^+ | i \in S_A \cap j \in S_B\}| \\
-|\{\{A,B\}\in P^- | i \in S_A \cap j \in S_B\}| &\text{if}~i \neq j \\ 
0 & \text{otherwise}.\\
\end{array}
\right. \label{eq:min_cost}
\end{equation}
Thus, we can reconstruct the original node connection info by counting the edges between the ancestor node set of leaf nodes i and j.




\smallsection{Encoding cost:} \label{encodingCost}As in the previous studies \cite{beg2018scalable, shin2019sweg}, we store an output summary graph in an edge list format. Thus, we measure the size of the output hierarchical summary graph by the number of superedges (i.e., $|P^+|$ and $|P^-|$), including h-edges \hieredge. Therefore, the encoding cost is as follows:
\begin{align}
Cost(\overline{G}) := |P^+| + |P^-| + |H|.
\label{eq:encodingCost}
\end{align}
Similarly, the input graph's encoding cost and the summary graph are $Cost(G) := |E|$ and $Cost(\tilde{G}) := |C^+| + |C^-| + |P| + |H|$, respectively.

\subsection{Problem Definition}
Now that we have defined necessary notations and concepts, we formally introduce hierarchical graph summarization problem. Then, we compare the difference between our new hierarchical model and the previous graph summarization model. 
\begin{problem}[\label{problem}Hierarchical Graph Summarization]~
	\begin{itemize}[leftmargin=*]
		\item \textbf{Given:} an input graph \original
		\item \textbf{Find:} a hierarchical summary graph \sG
		\item \textbf{to Minimize:} $Cost(\overline{G}) := |P^+| + |P^-| + |H|$ (Eq.~(\ref{eq:encodingCost})).
	\end{itemize}
\end{problem}
\smallsection{Comparison with the original model:} Original graph summarization model summarizes an input graph \original into \summary and corrections \correction, where $P$ is a set of superedges that connect supernodes and \correction is sets of subedges that connect subnodes. Thus, it couldn't represent an input graph with connections between supernode and subnodes (Constraint on node connection).

The root node in the hierarchical summarization model denotes a node that does not have a larger superset that includes all the child's leaf descendants, which in the previous model is supernode. Also, the leaf node in the hierarchical summarization model directly corresponds to subnodes. Thus, an internal node did not exist in the previous model (Absence of various nodes). However, with the expense of additional h-edges \hieredge connecting the internal node and its parent.

Due to these advantages, the hierarchical graph summarization model can connect nodes without any constraints, thus representing an input graph with various node connections. Moreover, note that the previous graph summarization model is a special case of the hierarchical graph summarization model. Illustration of the hierarchical graph summmarization is in the following example \red{Fig.~\ref{fig:model}}.

